Differentiable Optimization Based Time-Varying Control Barrier Functions for Dynamic Obstacle Avoidance

Control barrier functions (CBFs) provide a simple yet effective way for safe control synthesis. Recently, work has been done using differentiable optimization (diffOpt) based methods to systematically construct CBFs for static obstacle avoidance tasks between geometric shapes. In this work, we extend the application of diffOpt CBFs to perform dynamic obstacle avoidance tasks. We show that by using the time-varying CBF (TVCBF) formulation, we can perform obstacle avoidance for dynamic geometric obstacles. Additionally, we show how to extend the TVCBF constraint to consider measurement noise and actuation limits. To demonstrate the efficacy of our proposed approach, we first compare its performance with a model predictive control based method and a circular CBF based method on a simulated dynamic obstacle avoidance task. Then, we demonstrate the performance of our proposed approach in experimental studies using a 7-degree-of-freedom Franka Research 3 robotic manipulator.

==> proof.tex <==
We now show that with the scheme proposed above a probability bound can be given on satisfaction of the TVCBF constraint. Using the CBF in~\eqref{eq:diff_opt_cbf}, the TVCBF constraint in~\eqref{eq:tvcbfqp} can be written as
\begin{equation}
    \dot{\alpha} \geq -\gamma(\alpha - \beta).
\end{equation}
This constraint guarantees, instantaneously, that $\alpha \geq \beta$. Thus, for any $\Tilde{\alpha} \geq \alpha$, we have $\Tilde{\alpha} - \beta \geq 0$. Let the CBF for the actual obstacle be $\Tilde{\alpha} - \beta$ and the CBF for the virtual obstacle that has the smallest CBF value in the $k\sigma$ region be $\hat{\alpha} - \beta$. Note that for any obstacle configuration in the $k\sigma$ region, it will have a larger CBF value than $\hat{\alpha} - \beta$. Thus, using the reasoning above we can see that if we can guarantee safety with respect to this virtual obstacle, then we can guarantee safety with respect to any obstacle configuration in the $k\sigma$ region. Thus, we can obtain a lower bound on the probability that safety is guaranteed
\begin{equation}
    \mathrm{Prob}(\mathrm{Safe}) \geq \mathrm{Prob}(k\sigma)
\end{equation}

\begin{rem}
Finding the configuration that gives us $\hat{\alpha}$ is a nonlinear program that is computationally expensive to solve. Therefore, we have provided a heuristic-based approach to find an estimation of the configuration that gives us an estimation of $\hat{\alpha}$ which is simple to implement and is computationally very cheap.    
\end{rem}
